Learning Efficient Abstract Planning Models that Choose What to Predict

An effective approach to solving long-horizon tasks in robotics domains with continuous state and action spaces is bilevel planning, wherein a high-level search over an abstraction of an environment is used to guide low-level decision-making. Recent work has shown how to enable such bilevel planning by learning abstract models in the form of symbolic operators and neural samplers. In this work, we show that existing symbolic operator learning approaches fall short in many robotics domains where a robot's actions tend to cause a large number of irrelevant changes in the abstract state. This is primarily because they attempt to learn operators that exactly predict all observed changes in the abstract state. To overcome this issue, we propose to learn operators that 'choose what to predict' by only modelling changes necessary for abstract planning to achieve specified goals. Experimentally, we show that our approach learns operators that lead to efficient planning across 10 different hybrid robotics domains, including 4 from the challenging BEHAVIOR-100 benchmark, while generalizing to novel initial states, goals, and objects.

==> acknowledgements.tex <==
\section*{Acknowledgements}
We gratefully acknowledge support from NSF grant 2214177; from AFOSR grant FA9550-22-1-0249; from ONR MURI grant N00014-22-1-2740; from ARO grant W911NF-23-1-0034; from the MIT-IBM Watson Lab; and from the MIT Quest for Intelligence.
Nishanth, Willie, and Tom are supported by NSF Graduate Research Fellowships.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of our
sponsors.
We thank Jorge Mendez and Aidan Curtis for helpful comments on earlier drafts of this work.

==> bilevelplanning.tex <==
\paragraph{Bilevel Planning with Operators}
\label{sec:bilevel-planning}

\begin{wrapfigure}{H}{0.45\textwidth}
\begin{minipage}{0.5\textwidth}
    \vspace{-1.5em}
    \begin{algorithm}[H]
      \SetAlgoNoEnd
      \DontPrintSemicolon
      \SetKwFunction{algo}{algo}\SetKwFunction{proc}{proc}
      \SetKwProg{myalg}{}{}{}
      \SetKwProg{myproc}{Subroutine}{}{}
      \SetKw{Continue}{continue}
      \SetKw{Break}{break}
      \SetKw{Return}{return}
    \myalg{\textsc{PreimageBackchaining(}($\operators$,$(\statetraj, \plan), \objects, \goal$){)}}{
        \nl $n \gets \text{length}(\statetraj)$\;
        \nl $\necessaryatoms_n \gets \goal$\;
        \nl \For{$i \gets n-1, n-2, \dots, 0$}
        {
            \nl $\abstractstate_i, \abstractstate_{i+1} \gets \textsc{Abstract}(x_i), \textsc{Abstract}(x_{i+1})$\;
        \nl $\ground{\operator}_{\text{best}} \gets$ \textsc{FindBestConsistentOp}($\operators$, $\abstractstate_i$, $\abstractstate_{i+1}$, $\necessaryatoms_{i+1}$, $\objects$)\;
        \nl \If{$\ground{\operator}_{\text{best}} = \text{Null}$}
        {
            \Break
        }
        \nl $\ground{\operator_{i+1}} \gets \ground{\operator}_{\text{best}}$\;
        \nl $\necessaryatoms_i \gets  \ground{\preconditions_{i + 1}} \cup (\necessaryatoms_{i+1} \setminus \ground{\addeffects_{i+1}})$\;
       
        }
        \nl \Return{$(\ground{\operator_{i+1}}, \ldots, \ground{\operator_{n}}), (\necessaryatoms_i, \ldots, \necessaryatoms_n)$}
        }\;
    \caption{Pseudocode for our preimage backchaining procedure.}
    \label{alg:backchaining}
    \caption{\small{Pseudocode for our preimage backchaining algorithm. The inputs are a set of operators $\operators$, a training demonstration $(\statetraj, \plan)$, objects used in the corresponding task $\objects$, and the task goal $\goal$. The output is an abstract plan suffix $(\ground{\operator_{i+1}}, \ldots, \ground{\operator_{n}})$ and corresponding sequence of necessary atoms $(\necessaryatoms_i, \ldots, \necessaryatoms_n)$. Intuitively, we pass backward through each transition in a trajectory while attempting to choose an operator in $\operators$ to ``cover'' the transition and then updating the transition's necessary atoms using Definition \ref{def:necessary-atoms}. 
    If multiple such operators exist, we use a heuristic that attempts to select the one that best matches the transition (see Appendix \ref{appendix:data-partitioning} for details).}}
    \end{algorithm}
    \vspace{-1.5em}
\end{minipage}
\end{wrapfigure}

Given planning operators learned from training tasks $\traintasks$, we can solve new evaluation tasks $\task \in \tasks$ via search-then-sample bilevel planning (Algorithm~\ref{alg:bilevel}).
We provide a brief review of bilevel planning and refer to Appendix \ref{appendix:bilevel-planning} and previous works for details~\citep{garrett2021integrated, chitnis2021learning,LOFT2021,silver2022learning,silver2022inventing}.
Given the task goal $\goal$, initial state $\initstate$, and corresponding abstract state $\abstractstate_0 = \abstractfn(\initstate)$, bilevel planning uses efficient AI planning techniques (e.g., \citep{helmert2006fast}) to generate candidate \emph{abstract plans}.
An abstract plan is a sequence of ground operators $(\ground{\operator}_1, \dots, \ground{\operator}_{n})$ where 
$g \subseteq \abstractstate_n$ and $\abstractstate_{i} = \abstracttransitionfn(\abstractstate_{i-1}, \ground{\operator}_i)$ for $1 \le i \le n$.
The corresponding abstract state sequence $(\abstractstate_1, \dots, \abstractstate_{n})$ serves as a sequence of \emph{subgoals} for low-level planning.
Furthermore, the operator controller sequence $(\ground{\controller}_1, \dots, \ground{\controller}_{n})$ provides a \emph{plan sketch}, where all that remains is to \textit{refine} the plan by ``filling in'' the continuous parameters.
We do this by sampling continuous parameters $\theta$ for each controller starting from the first and checking if the controller achieves its corresponding subgoal $\abstractstate_i$. If we cannot sample such parameters within a constant budget, we backtrack and resample, eventually even generating a new abstract plan.
Following previous work~\citep{chitnis2021learning}, we use learned neural network samplers to propose continuous controller parameters (see Appendix \ref{appendix:samplers} for more details).
Importantly, note that bilevel planning is capable of generating \textit{multiple} abstract plans. Thus, the operators need not guarantee yielding abstract plans that are \textit{downward refinable}, as is typically assumed in works that learn operators for classical planning (e.g. ~\citet{drescher1991made, amir2008learning, kruger2011object}).


% Starting with the first controller $\ground{\controller}_1$, we repeatedly sample parameters $\theta$ until the corresponding subgoal $\abstractstate_1$ is achieved, i.e., $\abstractfn(\state_1) \subseteq \abstractstate_1$ where $\state_1 = \transitionfn(\state_0, \action_1)$ and $\action_1 = \ground{\controller}_1(\theta)$.
% We then continue onto sampling parameters for $\ground{\controller}_2$ from $\state_1$ to reach $\abstractstate_2$, and so on, until the task goal is achieved.
% If at any step a constant sampling budget is exceeded, we backtrack and resample previous controllers.
% If we backtrack to the beginning, we discard the abstract plan and continue on to the next abstract plan, repeating this process until a global timeout is exceeded or a maximum number of abstract plans are considered.
% As described, this planning strategy is incomplete, but it is possible to ensure completeness with minor modifications that revisit all abstract plans infinitely many times in the limit~\citep{dantam2016incremental}.

% For example, if we had two operators per controller --- one operator with empty preconditions and effects, and another operator with empty preconditions and add effects for achieving the goal --- we may technically satisfy completeness, but the operators would be far too general to helpfully constrain sampling.
% On the other hand, if we created one operator to exactly match every transition seen in data, we would have very specific samplers, but at the expense of feasibility, since applying the transition-specific operators in new problems would frequently fail.
% In the following section, we show how operators learned by optimizing prediction error can lead to over-specificity and frequent infeasibility in natural settings.
% We then propose an alternative objective for operator learning to remedy this issue.

% \textbf{TODO: Similar to predicate-invention and LOFT papers, describe bilevel planning in more detail.}
% \begin{itemize}
%     \item Describe how high-level plans are generated via traditional A* search/any classical planning approach.
%     \item Describe how these are then refined (need to define samplers here).
%     \item Mention backtracking process.
%     \item Specifically highlight how - for refinement to succeed - the atoms predicted by high-level planning must be correct.
% \end{itemize}


==> limitations.tex <==
\section{Limitations}
\label{sec:limitations}
Our method assumes that the provided predicates $\predicates$ comprise a good state abstraction given the task distribution for operator learning. With completely random or meaningless predicates, our approach is likely to learn very complex operators such that planning with these is unlikely to outperform non-symbolic behavior-cloning baselines.
Fortunately, prior work~\citep{silver2022inventing} suggests such `good' predicates can themselves be learned from data.
There is no guarantee that our overall hill-climbing procedure will converge quickly; the \textsc{ImproveCoverage} successor generator is especially computationally expensive to run. In practice, we find its learning time to be comparable or faster than baseline methods in our domains (\secref{appendix:additional-experiments} in the appendix), though this may not hold in more complex domains where a very large (e.g. greater than 100) number of operators need to be learned.
Additionally, our \textsc{ImproveCoverage} successor generator is rather complicated, and there is perhaps a simpler way to achieve the same desiderata (i.e, generating a new operator set that is guaranteed to decrease the \texttt{coverage} term of our objective).
